Beam-induced and cosmic-ray backgrounds observed in the ATLAS detector during the LHC 2012 proton-proton running period

This paper discusses various observations on beam-induced and cosmic-ray backgrounds in the ATLAS detector during the LHC 2012 proton-proton run. Building on published results based on 2011 data, the correlations between background and residual pressure of the beam vacuum are revisited. Ghost charge evolution over 2012 and its role for backgrounds are evaluated. New methods to monitor ghost charge with beam-gas rates are presented and observations of LHC abort gap population by ghost charge are discussed in detail. Fake jets from colliding bunches and from ghost charge are analysed with improved methods, showing that ghost charge in individual radio-frequency buckets of the LHC can be resolved. Some results of two short periods of dedicated cosmic-ray background data-taking are shown; in particular cosmic-ray muon induced fake jet rates are compared to Monte Carlo simulations and to the fake jet rates from beam background. A thorough analysis of a particular LHC fill, where abnormally high background was observed, is presented. Correlations between backgrounds and beam intensity losses in special fills with very high $\beta^*$ are studied.

==> boostedsymbols.tex <==
%
% User-defined latex commands for SUBSTRUCTURE
%

\RequirePackage{xspace}


% Jet mass related
\newcommand{\mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\mlead}     {\ensuremath{\mjet_{1}}\xspace}
\newcommand{\mleadavg}  {\ensuremath{\langle\mlead\rangle}\xspace}
\newcommand{\Mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\massjet}   {\mjet}
\newcommand{\mjetAvg}   {\ensuremath{\langle\mjet\rangle}\xspace}
\newcommand{\masstrkjet}{\ensuremath{m^{\rm track \; jet}}\xspace}

% Particle (and mass) related
\newcommand{\Wmass}     {\ensuremath{m_{\Wboson}}\xspace}
\newcommand{\WmassT}    {\ensuremath{m^{\Wboson}_{T}}\xspace}
\newcommand{\topmass}   {\ensuremath{m_{\rm top}}\xspace}
\newcommand{\massZprime}{\ensuremath{m_{\Zprime}}\xspace}

% Jet algorithm and grooming related
\newcommand{\akt}       {\antikt\xspace}
\newcommand{\Akt}       {\Antikt\xspace}
\newcommand{\aktfour}    {\antikt, \ensuremath{R=0.4}\xspace}
\newcommand{\aktsix}    {\antikt, \ensuremath{R=0.6}\xspace}
\newcommand{\aktten}    {\antikt, \ensuremath{R=1.0}\xspace}
\newcommand{\AKTFat}    {\antikt, \ensuremath{R=1.0}\xspace}
\newcommand{\AKTPrune}  {\antikt, \ensuremath{R=1.0} (pruned)\xspace}
\newcommand{\AKTFilt}   {\antikt, \ensuremath{R=1.0} (filtered)\xspace}
\newcommand{\KTSix}     {\ensuremath{k_{t}}, \ensuremath{R=0.6}\xspace}
\newcommand{\kt}        {\ensuremath{k_{t}}\xspace}
\newcommand{\ca}        {Cambridge-Aachen\xspace}
\newcommand{\CamKt}     {\ensuremath{\mathrm{C/A}}\xspace}
\newcommand{\CASix}     {\CamKt, \ensuremath{R=0.6}\xspace}
\newcommand{\CAFat}     {\CamKt, \ensuremath{R=1.2}\xspace}
\newcommand{\CAPrune}   {\CamKt, \ensuremath{R=1.2} (pruned)\xspace}
\newcommand{\CAFilt}    {\CamKt, \ensuremath{R=1.2} (filtered)\xspace}
\newcommand{\SISCone}   {SISCone}
\newcommand{\SISConeSiz}{\SISCone, \ensuremath{R=0.6}\xspace}
\newcommand{\minKt}     {\ensuremath{\min\left(\pti^2, \ptj^2\right)}\xspace}
\newcommand{\minAKt}    {\ensuremath{\min\left(\pti^{-2}, \ptj^{-2}\right)}\xspace}
\newcommand{\minGen}    {\ensuremath{\min\left(\pti^{2p}, \ptj^{2p}\right)}\xspace}
\newcommand{\Rij}       {\ensuremath{R_{ij}}\xspace}
\newcommand{\DRij}      {\ensuremath{\Delta\Rij}\xspace}
\newcommand{\DRratio}   {\ensuremath{\frac{(\DRij)^2}{R^2}}\xspace}
\newcommand{\diB}       {\ensuremath{d_{iB}}\xspace}
\newcommand{\Rfilt}     {\ensuremath{R_{\rm filt}}\xspace}
\newcommand{\sjone}     {\ensuremath{j_{1}}\xspace}
\newcommand{\sjtwo}     {\ensuremath{j_{2}}\xspace}
\newcommand{\msubjone}  {\ensuremath{m^{\sjone}}\xspace}
\newcommand{\msubjtwo}  {\ensuremath{m^{\sjtwo}}\xspace}
\newcommand{\ptsubjone} {\ensuremath{p_{T}^{\sjone}}\xspace}
\newcommand{\ptsubjtwo} {\ensuremath{p_{T}^{\sjtwo}}\xspace}
\newcommand{\Rsubjets}  {\ensuremath{R_{\sjone,\sjtwo}}\xspace}
\newcommand{\DRsubjets} {\ensuremath{\Delta\Rsubjets}\xspace}
\newcommand{\Nsubjet}   {\ensuremath{N_{\rm subjet}}\xspace}
\newcommand{\pti}       {\ensuremath{p_{Ti}}\xspace}
\newcommand{\ptj}       {\ensuremath{p_{Tj}}\xspace}
\newcommand{\ycut}      {\ensuremath{y_{\rm cut}}\xspace}
\newcommand{\mcut}      {\ensuremath{m_{\rm cut}}\xspace}
\newcommand{\ymin}      {\ensuremath{y_{\min}}\xspace}
\newcommand{\fcut}      {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}      {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\drsub}     {\ensuremath{\Rsub}\xspace}
\newcommand{\mufrac}    {\ensuremath{\mu_{\rm frac}}\xspace}
\newcommand{\rcut}      {\ensuremath{R_{\rm cut}}\xspace}
\newcommand{\zcut}      {\ensuremath{z_{\rm cut}}\xspace}
\renewcommand{\pt}      {\ensuremath{p_{\rm T}}\xspace}
\renewcommand{\pttrue}  {\ensuremath{p_{\rm T}^{\rm true}}\xspace}
\newcommand{\largeR}    {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}    {Large-\ensuremath{R}\xspace}


% Insitu mass validation
\newcommand{\rtrkjet}       {\ensuremath{r_{\rm track \; jet}}\xspace}
\newcommand{\rtrkjetPt}     {\ensuremath{\rtrkjet^{p_T}}\xspace}
\newcommand{\rtrkjetM}      {\ensuremath{\rtrkjet^{m}}\xspace}
\newcommand{\AvgrtrkjetM}   {\ensuremath{\langle\rtrkjet^{m}\rangle}\xspace}
\newcommand{\rtrkjetPtData} {\ensuremath{\rtrkjet^{p_{T},{\rm data}}}\xspace}
\newcommand{\rtrkjetMData}  {\ensuremath{\rtrkjet^{m,{\rm data}}}\xspace}
\newcommand{\rtrkjetPtMC}   {\ensuremath{\rtrkjet^{p_{T},{\rm MC}}}\xspace}
\newcommand{\rtrkjetMMC}    {\ensuremath{\rtrkjet^{m,{\rm MC}}}\xspace}
\newcommand{\RtrkjetPt}     {\ensuremath{R_{r{\rm \; track \; jet}}^{p_T}}\xspace}
\newcommand{\RtrkjetM}      {\ensuremath{R_{r{\rm \; track \; jet}}^{m}}\xspace}

% Jet substructure related
\newcommand{\subjetpt}  {\ensuremath{p_{T}^{\rm subjet}}\xspace}
\newcommand{\yij}       {\ensuremath{y_{ij}}\xspace}
\newcommand{\dcut}      {\ensuremath{d_{\rm cut}}\xspace}
\newcommand{\dmin}      {\ensuremath{d_{\min}}\xspace}
\newcommand{\dij}       {\ensuremath{d_{ij}}\xspace}
\newcommand{\Dij}       {\ensuremath{\sqrt{\dij}}\xspace}
\newcommand{\DOneTwo}   {\ensuremath{\sqrt{d_{12}}}\xspace}
\newcommand{\DTwoThr}   {\ensuremath{\sqrt{d_{23}}}\xspace}
\newcommand{\xj}        {\ensuremath{x_{J}}\xspace}
\newcommand{\jetFunc}   {\ensuremath{J^{(eik),c} (\mjet,\pT,R)}\xspace}
\newcommand{\tauN}      {\ensuremath{\tau_N}\xspace}
\newcommand{\tauTwoOne} {\ensuremath{\tau_{21}}\xspace}
\newcommand{\tauThrTwo} {\ensuremath{\tau_{32}}\xspace}
\newcommand{\dip}       {\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dipOneTwo} {\ensuremath{\dip_{12}}\xspace}
\newcommand{\dipTwoThr} {\ensuremath{\dip_{23}}\xspace}
\newcommand{\dipOneThr} {\ensuremath{\dip_{13}}\xspace}

% Samples
\newcommand{\Zprimett}  {\ensuremath{Z'\ra t\bar{t}}\xspace}
\newcommand{\Zqq}       {\ensuremath{Z\ra q\bar{q}}\xspace}
\newcommand{\Wqq}       {\ensuremath{W\ra q\bar{q}}\xspace}


% Random
\newcommand{\mpi}       {multiple parton interactions\xspace} % David/Emily using multiple proton interactions.

\newcommand{\DRmin}     {\ensuremath{\Delta{R}_{min}}\xspace}

\newcommand{\avg}[1]{\left< #1 \right>} % for e.g. <\mu>
                                                                                                                 


==> lucid.tex <==
\section{Background monitoring with the LUCID detector}
\label{sect:lucid}

The LUCID subdetector was introduced as a dedicated luminosity monitor. It consists of
16 Cherenkov tubes, each connected to its own photomultiplier (PMT). In 2012 LUCID was most
of the time operated without gas in the tubes, and only the Cherenkov light from the
PMT-window was used for particle detection.  
The LUCID subdetectors are situated in the forward region at $\eta=5.6-6.0$ and $z=18.3$\,m 
(PMT-windows) from the IP. 

The LUCID data are recorded by the luminosity data-acquisition software independently of
the ATLAS trigger and is available per bunch and luminosity block with typically very good
statistics.


The LUCID detector is not as fast as the BCM and suffers more from afterglow.
Unlike in 2011, the 2012 operation had two specific cases where LUCID proved very 
useful to detect backgrounds, although used in a way it was never
intended. These were the high-$\beta^*$ fills with very low luminosity and sparse bunch 
pattern and a normal fill with abnormally high background. Both will be discussed
in detail later.

Of particular importance for this method is the large distance from the IP, which allows to
separate the background signal from luminosity and related afterglow.
The usable signal comes from the background associated with the incoming bunch, observed in the upstream LUCID. 
The incoming bunch passes the upstream detector about 60\,ns before the actual collision which means that
the signal of background associated with that bunch appears 5 BCID before the luminosity signal. This is 
illustrated in figure\,\ref{fig:lucidearly}.
Unlike the one-sided BCM signal, this early LUCID signal has practically no luminosity contamination
even in paired bunches and yields itself very well to monitor the beam background -- but only of bunches 
with a long empty gap preceding them.

In a normal physics bunch pattern the only bunches for which this method can in principle be applied 
are the first three unpaired in BCIDs 1, 3 and 5, which for most of the year were in beam-1 and the first three bunches of 
the first  paired train, i.e. bunches in BCIDs 66, 68 and 70. Even for these six BCIDs the background, at its
the normal level, is overwhelmed by the afterglow in a normal physics fill. 


\begin{figure}[t]
\centering 
\includegraphics[width=\textwidth]{lucidearly.pdf}
\caption{Background and luminosity signal seen by LUCID in the high-$\beta^*$ fill (discussed in Section\,\protect\ref{sect:highbeta}). 
Particular characteristics of this fill were a very low bunch-luminosity and the presence of only 3 well-separated bunches per beam.
The normal luminosity signal appears in BCID 1886 and is of similar size during high beam losses and in normal background conditions. The
background signal appears five BCID earlier and peaks in BCID 1881. In during normal beam losses it is much smaller
than the luminosity peak, but during high losses (see Section\,\protect\cite{sect:highbeta}) it can become very prominent. Both 
data-sets average over three ATLAS luminosity blocks, i.e. about 180\,s.}
\label{fig:lucidearly}
\end{figure}



